The phase transition for the three-state SOS model with one-level competing interactions on the binary tree

In this paper, we consider a three-state solid-on-solid (SOS) model with two competing interactions (nearest-neighbour, one-level next-nearest-neighbour) on the Cayley tree of order two. We show that at some values of parameters the model exhibits a phase transition. We prove that for the model under some conditions there is no antiferromagnetic phases.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{rs} Rozikov, U.A., Suhov, Yu.M.: Gibbs measures for SOS model on a Cayley tree. Inf. Dim. Anal. Quant. Prob. Rel. Fields. V.9, No.3, p.471-488.,(2006), https://doi.org/10.1142/S0219025706002494

\bibitem{7} Sinai, Ya. G.: Theory of phase transitions: rigorous results. Pergamon Press, Oxford (1982)

\bibitem{B} Preston,C. J.: Gibbs States on Countable Sets, Cambridge University Press, London (1974)

\bibitem{B1} Blekher, P.M.,  Ganikhodzhaev, N.N.:  On pure phases of the Ising model on the Bethe lattices. Teor. Veroyatnost. i Primenen., 35:2 (1990), 220230; Theory Probab. Appl., 35:2, 216-227, (1990)

\bibitem{B2} Bleher, P.M., Ruiz, J., Zagrebnov, V.A.: On the purity of the limiting gibbs state for the Ising model on the Bethe lattice. J Stat Phys 79, 473-482 (1995). https://doi.org/10.1007/BF02179399

\bibitem{B3} K\"{u}lske, C., Rozikov, U.A.: Fuzzy transformations and extremality of Gibbs measures for the potts model on a Cayley tree, Random Structures and Algorithms. (2016) https://doi.org/10.1002/rsa.20671

\bibitem{8} Ganikhodjaev, N.N., Rozikov, U.A.: Description of periodic extreme Gibbs measures of some lattice model on the Cayley tree. Theor. and Math. Phys. V. 111, No 1, p.480-486. (1997) DOI: https://doi.org/10.4213/tmf993

\bibitem{Ro} U. A. Rozikov, Gibbs Measures on Cayley Trees, World Scientific, Singapore, 2013.

\bibitem{re} Rozikov, U.A.: On $q$-Component Models on Cayley Tree: Contour Method. Lett. Math. Phys. 71, 27-38 (2005). https://doi.org/10.1007/s11005-004-5117-2

\bibitem{zo} Zimmer, W. M., Obermair,G. M.: Spherical model on the Cayley tree, (1978) J. Phys. A: Math. Gen. 11 1119, DOI: 10.1088/0305-4470/11/6/022

\bibitem{G} Georgii, H.O.: Gibbs Measures and Phase Transitions. W. de Gruyter, Berlin (1988).

\bibitem{Zach} Zachary, S.: Countable state space Markov random fields and Markov chains on trees, Ann. Probab. 11 (1983) 894-903. doi: 10.1214/aop/1176993439

\bibitem{Zach2} Zachary,S.: Bounded, attractive and repulsive Markov specifications on trees and on the one-dimensional lattice, Stochastic Processes and their Applications. (1985) https://doi.org/10.1016/0304-4149(85)90213-3

\bibitem{NNG} Ganikhodjaev, N.N., Mukhamedov, F.M., Mendes, J.F.F.: On the three state Potts model with competing interactions on the Bethe lattice, Jour. Stat. Mech. 2006, P08012, 29 p, doi:10.1088/1742-5468/2006/08/P08012

\bibitem{MF} Mukhamedov, F.: On factor associated with the unordered phase of $\lambda-$model on a Cayley tree. Rep. Math. Phys. 1-18,53 (2004)

\bibitem{Pah} Mukhamedov, F., Pah, C.H., Jamil, H., Rahmatullaev, M.: On ground states and phase Transition for $\lambda-$model with the competing Potts interactions on Cayley trees, Physica A 549 (2020), 124184., https://doi:10.1016/j.physa.2020.124184

\bibitem{2}  Mazel, A.E., Suhov, Y.M.: Random surfaces with two-sided constraints: An application of the theory of dominant ground states. J. Stat. Phys. 64, 111-134 (1991). https://doi.org/10.1007/BF01057870

\bibitem{Kelly} Kelly, F.P.:  Stochastic models of computer communication systems. With discussion, J. Roy. Statist. Soc. Ser. B 47 (1985) 379-395;  https://doi.org/10.1111/j.2517-6161.1985.tb01367.x

\bibitem{Raman} Ramanan, K., Sengupta, A., Ziedens, I., Mitra,P.: Markov random field models of multicasting in tree networks, Advances in Applied Probability. (2002)  https://doi.org/10.1239/aap/1019160950

\bibitem{shok} Rozikov, U.A., Shoyusupov, S.A.:Gibbs measures for the SOS model with four states on a Cayley tree. Theor Math Phys 149, 13121323 (2006) https://doi.org/10.1007/s11232-006-0120-7

\bibitem{din} Dinaburg, E.I., Mazel, A.E.: Layering transition in SOS model with external magnetic field. J. Stat. Phys. 74, 533-563 (1994). https://doi.org/10.1007/BF02188570

\bibitem{KRSOS} Kuelske, C., Rozikov, U.A.: Extremality of Translation-Invariant Phases for a Three-State SOS-Model on the Binary Tree. J. Stat. Phys. 160, 659-680 (2015). https://doi.org/10.1007/s10955-015-1279-9

\bibitem{RH} Khakimov, R.M.: Localization of translation-invariant Gibbs measures for the Potts and solid-on-solid models on a Cayley tree. Theor Math Phys 179, 405415 (2014). https://doi.org/10.1007/s11232-014-0152-3

\bibitem{Muh} Rahmatullaev, M. M., Abdusalomova, M. R., Rasulova,M.A.: Ground states for the SOS model with an external field on the Cayley tree, Uzbek Math.Jour., 2020 No.2, 145-156, DOI:10.29229/uzmj.2020-2-14

\bibitem{Bun} Rahmatullaev,M.M., Abraev, B.U.: Non-translation invariant Gibbs measures of an SOS model on a Cayley tree. Reports on mathematical physics. Vol 86, No.3, (2020)  https://doi:10.1016/s0034-4877(20)30086-0

\bibitem{Bun2} Abraev, B.U.: On weakly periodic ground states for the SOS model, Scientific Bulletin of Namangan state university, No.3, 14-21. (2020)

\bibitem{sayg} Rahmatullaev, M.M., Rasulova, M.A.: Extremality Of Translation-Invariant Gibbs Measures
For The Potts-SOS Model On The Cayley Tree. J. Stat. Mech. (2021), https://doi.org/10.1088/1742-5468/ac08ff

\bibitem{mr} Rasulova, M.A.: Periodic Gibbs Measures for the Potts-SOS Model on a Cayley Tree. Theor. Math. Phys. 199, 586592 (2019). https://doi.org/10.1134/S0040577919040081

\bibitem{Bog} Bogachev, L.V., Rozikov, U.A.: On the uniqueness of Gibbs measure in the Potts model on a Cayley tree with external field. J. Stat. Mech. (2019) https://doi.org/10.1088/1742-5468/ab270b

\bibitem{potts} Rozikov, U.A.: Gibbs measures of Potts model on Cayley tree: a survey and applications, Reviews in Math. Phys., Vol. 33 (2021) 2130007, https://doi.org/10.1142/S0129055X21300077

\bibitem{Shir} Shiryaev, A.N.: Probability. Nauka, Moscow (1980).

\bibitem{k} Leung, K.T., Mok, I.A.C., Seun, S.N.: Polynomials and equations. Hong Kong University Press (1992.)


\end{thebibliography} 
